Automaton-Guided Control Synthesis for Signal Temporal Logic Specifications

This paper presents an algorithmic framework for control synthesis of continuous dynamical systems subject to signal temporal logic (STL) specifications. We propose a novel algorithm to obtain a time-partitioned finite automaton from an STL specification, and introduce a multi-layered framework that utilizes this automaton to guide a sampling-based search tree both spatially and temporally. Our approach is able to synthesize a controller for nonlinear dynamics and polynomial predicate functions. We prove the correctness and probabilistic completeness of our algorithm, and illustrate the efficiency and efficacy of our framework on several case studies. Our results show an order of magnitude speedup over the state of the art.

==> sections/Experiments.tex <==
\section{Evaluation}
\label{sec:experiments}
The objective of our evaluation is to analyze the efficacy of our automaton-guided approach for control synthesis under \stlnn specifications. We first illustrate the advantage of our framework in comparison benchmarks against related work \cite{stl-rrtstar} on linear and linearizable systems with linear predicates. Then, we show the impact of time partitioning on algorithm performance. Finally, we demonstrate the generality of our approach on a nonlinear system with polynomial predicates.

\subsection{Comparison Benchmarks}

We first consider the two systems in \cite{stl-rrtstar}, a 2D double integrator $\dot{x} = y$, $\dot{y} = u$
% \begin{align*}
%     \dot{x} = y, \quad \dot{y} = u
% \end{align*}
with a specification of 
\begin{align*}
    \varphi_1 = &\eventually_{[2,10]}(3.5 < x \leq 4 \wedge -0.2 < y \leq 0.2) \;\; \wedge \\& \globally_{[0,2]}(-0.5 < y \leq 0.5) \;\; \wedge \\& \globally_{[0,10]}((2 < x \leq 3) \rightarrow (y > 0.5 \vee x \leq -0.5)),
\end{align*}
and a second order unicycle system with dynamics
\begin{align*}
    \dot{x} = v \cos{(\phi)}, \quad
    \dot{y} = v \sin{(\phi)}, \quad \dot{\phi} = \omega,  \quad \dot{v} = a\text{,}
\end{align*}
with specification 
% $\varphi_2 = \eventually_{[0,18]}(3 < x \leq 4 \wedge 2 < y \leq 3) \wedge \globally_{[0,6]}\neg(1 < x \leq 2 \wedge 2 < y \leq 3).$
\begin{align*}
    \varphi_2 =& \eventually_{[0,18]}(3 < x \leq 4 \wedge 2 < y \leq 3) \;\; \wedge \\ 
               &\globally_{[0,6]}\neg(1 < x \leq 2 \wedge 2 < y \leq 3).
\end{align*}


We compared our approach to \cite{stl-rrtstar}, which we call STL-RRT*, another sampling based algorithm for STL that does not utilize automaton construction. We implemented both algorithms in the Open Motion Planning Library (OMPL) \cite{sucan2012the-open-motion-planning-library}. Table~\ref{tab:benchmarking} shows the time taken to compute a satisfying solution for both systems and specifications over $100$ trials, and the number of solutions found within the time limit of 30 seconds. It can be seen that our approach computes solutions considerably faster than STL-RRT*, with a success rate of $100\%$, whereas STL-RRT* can solve only $13\%$ of the instances for the unicycle model.  Additionally, we note that we use the full nonlinear dynamics for the unicycle model in our algorithm, while we need to use state-feedback linearization to ensure the availability of a steering function for both state and time (punctuality) for STL-RRT*. 
% \ri{we don't really have a "steering function" for time, but say it's good if it gets within epsilon of the goal in the time we give it. Don't have to rewrite if you think it's clear though}

\begin{table}
    \centering
    \caption{Benchmarking results, with a 30 second time limit. The success rate is the number of solutions computed within the time limit, and the mean time to first solution and standard deviation are reported.}
    \label{tab:benchmarking}
    \scalebox{0.96}{
    \begin{tabular}{l|c|c|c|c}
     & \multicolumn{2}{c|}{Double Integrator} & \multicolumn{2}{c}{Unicycle}\\
    % \hline
    Algorithm &  Succ. (\%) & Time (s) & Succ. (\%) & Time (s)\\\hline
    STL-RRT* & $\mathbf{100}$ & $1.83 \pm 0.12$ & $13$ & $7.51 \pm 0.71$ \\
    % \hline
    $\TA$-based & $\mathbf{100}$ & $\mathbf{1.10 \pm 0.02}$ & $\mathbf{100}$ &  $\mathbf{1.57 \pm 0.11}$
    \end{tabular}
    }
\end{table}
% \ri{might want to mention that this one works without a known steering function, though you are kind of implying that already}

% \ri{I don't know if we want to do/have time to do an analysis of the complexity of each algorithm, and if this one is better}

% Note that STL-RRT* assumes the availability of a steering function that solves the two point-boundary value problem in both state and time, an assumption that is restrictive.

\subsection{Impact of Time partitioning}

We study the benefits of varying the number of time partitions on the 2D double integrator with the following specification:
\begin{align*}
    \globally_{[0,t_1)} (x \leq 3.5 \wedge y \leq 3.5) \wedge \eventually_{[t_1,t_2]}(x > 3.5 \wedge y > 3.5),
\end{align*}
which forbids $x > 3.5$ and $y > 3.5$ until $t_1$, after which the system must eventually reach $x > 3.5, y > 3.5$ within the interval $[t_1, t_2]$. The minimal partition for this formula is $\{0,t_1\}$. We further partition the formula between $[0,t_1]$ to varying number of partitions $k$. The success rate and mean time to solution over 100 trials is reported in Table~\ref{tab:partitioning}, given a time limit of 30 seconds. 

\begin{table}[b]
    \centering
    \caption{Impact of time discretization, by varying the number of time partitions. The success rate is the number of solutions computed within the time limit (30 seconds), and the mean time to solution and standard deviation are reported.}
    \begin{tabular}{c|c|c}
    $k$ time partitions & Success (\%) & Time (s) \\\hline
    $1$ & $48$ & $3.77 \pm 0.64$\\
    $2$ & $81$ & $4.99 \pm 0.56$\\
    $\mathbf{5}$ & $\mathbf{100}$ & $\mathbf{4.42 \pm 0.51}$\\
    $15$ & $100$ & $8.35 \pm 0.32$\\
    $30$ & $100$ & $10.50 \pm 0.59$\\
    $50$ & $100$ & $8.89 \pm 0.50$\\
    $200$ & $51$ & $22.7 \pm 0.57$
    \end{tabular}
    \label{tab:partitioning}
\end{table}

The results show that varying these parameters affects the decomposition granularity of the constructed automaton in the time dimension, which directly impacts the computational efficiency of the algorithm. It can be seen that increasing the number of time partitions can improve the efficiency of solutions. This is due to the lead of the high-level layer being able to provide guides of finer granularity in the time dimension for the low-level layer. However, having too fine of a time granularity can lead to increased computation times, since the lead becomes harder for the low-level layer to follow.



\subsection{Nonlinear system and predicates}

To demonstrate the generality of our framework compared to previous approaches, we used our framework to synthesize a controller for the car-like nonlinear system presented in \cite{Webb2012KinodynamicRO}, with the following specification involving nonlinear predicates:
\begin{align*}
    \varphi_3 =& \globally_{[0,20.0]}((x - 5)^2 + (y-5)^2 > 2.0) \;\; \wedge \\
               & \eventually_{[0,20.0]}(x-10)^2 + y^2 < 2.0) \;\; \wedge \\ 
               & \eventually_{[0,10.0]}(x^2 + (y-10)^2 < 2.0).
\end{align*}
% \ri{if we end up having the space (doubt it), not a bad idea to write out the dynamics here as well}
Our algorithm computed a solution in less than $5$ seconds. Fig.~\ref{fig:nonlinearsystem} shows the resulting trajectory. In this figure $\globally_{[0,20.0]}((x - 5)^2 + (y-5)^2 > 2.0)$ is shown as a red circle, and $\eventually_{[0,20.0]}((x-10)^2 + y^2 ) < 2.0$ and $\eventually_{[0,10.0]}(x^2 + (y-10)^2 < 2.0)$ are shown as blue and green quadrants respectively. We emphasize that previous approaches cannot handle such a combination of nonlinear dynamics with input constraints and nonlinear predicates.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/nonlinearcar_trimmed.png}
    \caption{Resulting trajectory for $\varphi_3$ in blue. The system starts from the bottom left, and the controller drives it to the blue region at the top left within 10 seconds, and then to the green region within 20 seconds, while avoiding the red region.}
    \label{fig:nonlinearsystem}
    \vspace{-2mm}
\end{figure}
% \qh{- Section VI.C: The control input trajectory would be
% interesting to see.}

==> sections/Methodology.tex <==
\section{Temporal-aware Automata Guided Search}
% \section{TEMPORAL AWARE AUTOMATA GUIDED SEARCH}
\label{sec:method}

Here, we present our control synthesis framework that solves Problem~\ref{prob:controllersynthesis}. Our approach can be formalized by decomposing Problem~\ref{prob:controllersynthesis} into two steps: timed automaton construction and sampling-based search.
% \begin{problem}
%     \label{prob:hybridautomata}
%     Given an \stlnn formula $\varphi$, construct a timed NFA $\TA$ such that $(\mathbf{w}, \mathbf{t}) \in \mathcal{L}(\TA) \iff (\mathbf{w}, \mathbf{t}) \models \varphi$.
%     \ml{semantics of $\varphi$ are defined over trajectories, not timed words!}
% \end{problem}
We first observe that \stlnn formulas reason over a single (global) time. Taking advantage of this, we propose a novel algorithm to efficiently construct a timed NFA $\TA$ such that every trajectory that satisfies the \stlnn formula has a timed word that is accepted by $\TA$.
% \begin{problem}
%     \label{prob:final}
%     Given a timed NFA $\mathcal{A}$, synthesize a controller $\pu$ that drives System~\eqref{eq:system} through a timed path $(\mathbf{p}, \mathbf{t})$ whose timed word $w((\mathbf{p}, \mathbf{t}))$ satisfies $\varphi$.
% \end{problem}
Next, given $\TA$, our goal is to synthesize a controller $\pu$ that drives System~\eqref{eq:system} through a trajectory that satisfies $\varphi$. Note this is a reachability problem on the hybrid system that is induced from $\TA$ and System~\eqref{eq:system}. To efficiently solve this problem, we employ a sampling-based approach with high-level guides using an automaton. An overview of the algorithm is shown in Alg.~\ref{alg:framework}.

% Our approach to solve these subproblems has several components: (i) the construction of a timed automaton for the non-nested STL formula using time-partitioning (ii) Predicate Abstraction to decompose the state space based on the predicate functions and (iii) generation of a product automaton between the automaton and abstracted space to solve problem~\ref{prob:hybridautomata} and finally (iv) synergistic planning of discrete search over the product automaton to compute leads that guide a temporal sampling-based motion planner to synthesize a controller that satisfies the STL formula, to solve problem~\ref{prob:final}. The pseudocode for the framework is shown in Alg~\ref{alg:fullsearch}. \qh{TODO: Reword this paragraph} 
% \ml{no need to give all this info here!}


\begin{algorithm}
    \caption{Automaton-Guided Synthesis for STL}
    \label{alg:framework}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{STL$_{nn}$ formula $\varphi$, state space $X$, system dynamics $\dot{x}$, initial state $x_0$, time bound $t_{max}$, exploration time bound $t_{e}$.}
    \Output{Trajectory containing system states and high-level states, and controller, if successful; returns 'No Solution' otherwise.}
    $\mathcal{M} \leftarrow$ ComputeAbstraction$(X, \varphi.H)$ \\
    $\TA_\varphi \leftarrow$ ConstructAutomaton$(\varphi)$\\
    $\mathcal{P} \leftarrow \mathcal{M} \otimes \TA_\varphi$\\
    $\textsc{tr} \leftarrow$ InitializeTree($x_0$)\\
    \While{Time Elapsed $< t_{max}$}
    {
        $\mathbf{L} \leftarrow \{(d_i, q_i)\}_{i \geq 0} \leftarrow$ ComputeLead($\mathcal{P}, t_{max}$)\\
        $C \leftarrow$ ComputeAvailableProductStates($\textsc{tr}, \mathbf{L}$)\\
        $(\mathbf{v}, \mathbf{u}, \mathbf{t}) \leftarrow$ Explore($\mathbf{L}, \textsc{tr}, \mathcal{P}, X, t_{e}$)\\
        \If{$(\mathbf{v}, \mathbf{u}, \mathbf{t}) \neq \emptyset$}{
            \Return $(\mathbf{v}, \mathbf{u}, \mathbf{t})$
        }
    }
    \Return No Solution
\end{algorithm}
\vspace{-2mm}

% \begin{algorithm}
%     \label{alg:computelead}
%     \caption{Compute Lead}
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \Input{Product Automaton $\mathcal{P}$}
%     \Output{lead}
%     $w(e) \leftarrow$ Compute edge weights for all vertices in $\mathcal{P}$\\
%     $\{(d_i, z_i)\}_{i \geq 0} \leftarrow$ Dijkstra'sShortestPath($w(e)$)\\
%     \Return $\{(d_i, z_i)\}_{i \geq 0}$
% \end{algorithm}

% \begin{algorithm}
%     \caption{isValid}
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \Input{v}
%     \Output{Boolean}
%     \If{$v.t \notin d.T$}{
%         \Return False
%     }
%     \Return True
% \end{algorithm}

\subsection{State Predicate Abstraction}
\label{sec:abstraction}
To construct the timed NFA, we first establish a relationship between predicates and state labels. To this end, we abstract the system into a discrete model based on the predicates. Note that predicates in $\Predicate$ define a semi-algebraic set on $\realnumbers^n$ since every $h \in H$ is a polynomial function. Hence, bounded state space $X \subset \realnumbers^n$ can be partitioned into a set of disjoint regions $D$ (i.e., the pairwise intersection of every two $d, d' \in D$ is empty, and the union of all $d \in D$ is the state space $X$), such that the points in each region are predicate-truth invariant, i.e., have the same truth-value assignments of the predicates in $\Predicate$.  Formally, for a partition region $d \subseteq X$ and every two points $x,x' \in d$, $\predicate(x) = \predicate(x')$ for all $\predicate \in \Predicate$. Through predicate abstraction, each state $x \in X$ is associated with a subset of $\Predicate$, a symbol $\sigma \in \Sigma = 2^{\Predicate}$. 
% We define function $L : D \rightarrow 2^{\Predicate}$ as a labeling function for a state $x$ that assigns the predicates that are true at $x$.
We define $L : D \rightarrow 2^{\Predicate}$ to be a labeling function that assigns to $d \in D$ the predicates that are true for all $x \in d$.

Predicate abstraction can be achieved in multiple ways. For polynomial predicate functions, methods such as cylindrical algebraic decomposition \cite{Lindemann2007, schwartz1983} can be used to find decompositions for predicate invariance. Computing this decomposition has a worst-case complexity of doubly exponential in the dimension of the space. For linear predicate functions, there exist efficient algorithms, e.g., geometry-based conforming Delaunay triangulation, to construct partitions that respect the predicate boundaries.

After partitioning the space into regions with predicate-truth invariance, we use the geometric adjacency relation between the regions to construct an adjacency-based graph.  This abstraction graph is a tuple $\mathcal{M} = (D, E, \Predicate, L)$, where the set of discrete states is $D$, and an edge $(d, d') \in E$ exists if there is adjacency between $d \in D$ and $d' \in D$.
% , which can be computed from the above abstraction methods. 
% $\Predicate$ and $L$ have the same definitions as above.
% This abstraction model captures all possible transitions between adjacent regions.
% an \qh{assumption} that is reasonable since our planning framework ultimately disallows transitions that are unrealizable for the dynamics of the system.
Note that $\mathcal{M}$ captures all possible transitions between adjacent regions even though they may not be realizable by System~\eqref{eq:system}. Such transitions are implicitly ignored in the second planning step of our framework, described in Sec.~\ref{sec:planning}. This is an advantage of our approach since it drastically reduces the computational burden of constructing a highly accurate abstraction.
% \reviewer{The abstraction of the system M builds from
% the polynomial function does not depend on the dynamics of
% the system but only on the geometric proximity between the
% resulting semi-algebraic sets. This introduces a additional transitions not realizable by
% the system, introducing non-determinism in the automaton.
% Can you justify why your approach eliminates them in the
% second step more effectively than it could in the
% beginning?
% }
\subsection{Automaton Construction}

Here, we introduce a novel method to construct a timed NFA from \stlnn formulas. This construction takes advantage of the non-nested aspect of this fragment for syntactic separation, and uses techniques from automata theory to construct an automaton that is partitioned in the time dimension. 

\begin{algorithm}
    \caption{Construct Automaton}
    \label{alg:automatonconstruction}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{\stlnn formula $\varphi$, time partition set $\mathbf{T}$.}
    \Output{Timed NFA $\TA_{\varphi}$.}
    $\{\Phi_i\}_{\geq 0} \leftarrow$ TimePartition($\varphi, \mathbf{T}$)\\
    $\TA \leftarrow \emptyset$\\
    \For{$\Phi \in \{\Phi_i\}_{i \geq 0}$}
    {
        \For{$\psi_{(t_{j-1}, t_j]} \in \Phi$}{
            $\psi^j \leftarrow$ IgnoreTimeWindows($\psi_{(t_{j-1}, t_j]}$)\\
            $\mathcal{A}_j \leftarrow $ LTLf2DFA($\psi^j$)\\
            $\TA_j \leftarrow$ ConvertToTimedDFA($\mathcal{A}_{j}, \psi_{(t_{j-1}, t_j]}$)\\
            $\TA_{\varphi} \leftarrow$ ConnectDFA($\TA_{\varphi}, \TA_{j}$)
        }
    }
    \Return $\TA_\varphi$
\end{algorithm}

The algorithm is shown in Alg.~\ref{alg:automatonconstruction}. It takes an \stlnn formula $\varphi$ and time partition set $\mathbf{T}$, and returns a timed NFA.  We explain the steps of the algorithm below and use the following running example to clarify the key concepts.

\begin{example}[Reach-avoid]
    \label{ex:reachavoidstl}
    Consider a system with $X \subset \realnumbers^2$ and specification ``reach a goal region defined by $3 < x_1 \leq 4$ and $2 < x_2 \leq 3$ in the first 18 seconds while avoiding unsafe region $3 < x_1 \leq 4$ and $2 < x_2 \leq 3$ in the first 6 seconds":
    \begin{align*}
        \varphi_\text{RA} =& \eventually_{[0,18]}(3 < x_1 \leq 4 \wedge 2 < x_2 \leq 3) \;\; \wedge \\ &  \globally_{[0,6]} \neg (1 < x_1 \leq 2 \wedge 2 < x_2 \leq 3) \\
        =& \eventually_{[0,18]}(\predicate_1(\px)) \wedge \globally_{[0,6]} \neg (\predicate_2(\px)).
    \end{align*}
\end{example}


\subsubsection{Time partitioning}

% \qh{Note, closed and open intervals are still not handled properly. Should be an easy fix... :)}

Given $\varphi$, our goal is to obtain an equivalent formula in which subformulas depend only on a disjoint segment of time. We can use the following equivalence rule to perform a syntactic separation.

\begin{proposition}[STL Separation \cite{boundedmodelchecking}]
    \label{prop:stlseparation}
    A \textit{time separation} of $\varphi \until_{[a,b]}\varphi'$ at time $\tau \in [a, b]$ is given by:
    \begin{align*}
    \varphi \until_{[a,b]}\varphi' \equiv &\; \varphi \until_{[a,\tau)} \varphi'  \nonumber \\
    &\vee \Big( \globally_{[a,\tau)} \varphi \wedge \big( \eventually_{[\tau,\tau]}(\varphi \wedge \varphi') \vee \varphi \until_{(\tau, b]}\varphi' \big) \Big).
\end{align*}

\end{proposition}
\noindent
Note that Proposition~\ref{prop:stlseparation} focuses on $\varphi \until_{[a,b]}\varphi'$, where $I = [a,b]$ is a closed time interval. Other cases of $I = \la a, b \ra$ are not shown but can be derived in a similar manner. 

We use this equivalence rule to syntactically separate the \stlnn formula $\varphi$ into $k$ time partitions, at time points in $\mathbf{T} = \{0,\tau_1, \cdots, \tau_{k-1}\}$ to obtain $k$ subformulas $\varphi_1, \cdots, \varphi_k$. We then express the partitioned formula in Disjunctive Normal Form (DNF) and obtain $\varphi = \Phi_1 \vee \Phi_2 \vee \cdots \vee \Phi_n$, where $\Phi_i, i \in \{1, \cdots, \Phi_n\}$ are clauses of DNF $\varphi$.
% \ml{expensive - (CNF to DNF) exponential}

The role of syntactic separation is to reformulate $\varphi$ into time discretized subformulas. By syntactically separating a formula into multiple sub-formulas connected by time, we are able to capture an increased time granularity in the timed NFA as discussed in Sec.~\ref{sec:experiments}.

We define the minimal time partition as the minimum number of partitions necessary to ensure that the time intervals are equivalent for all temporal operators in each subformula of $\Phi_i$. Note that this can always be achieved because of the non-nested property of \stlnn.
% \qh{Need a more robust way of defining this minimal time partition, what does equivalent mean?}

\begin{definition}[Minimal Time Partition]
    Let $T$ be the set of boundary points of the time intervals of the temporal operators in $\varphi$. The minimal time partition points is $\mathbf{T} = T \setminus \max(T)$.
\end{definition}

\begin{example}
\label{ex:subformulas}
Consider $\varphi_\text{RA}$ in Example~\ref{ex:reachavoidstl}. Using syntactic separation, we can separate each subformula at time $\mathbf{T} = \{0,6\}$ to form the minimal time partition, and with straightforward manipulation, we obtain the following formula in DNF form:
    $\varphi_\text{RA} = \Phi_1 \vee \Phi_2 \vee \Phi_3,$
    % \begin{equation*}
    %     \varphi = \Phi_1 \vee \Phi_2 \vee \Phi_3,
    % \end{equation*}
    where 
    \begin{align*}
        \Phi_1 =    & \eventually_{[0,6]}(\predicate_1(\px)) \wedge \globally_{[0,6]}\neg (\predicate_2(\px)), \\
        \Phi_2 =    &  \globally_{[0,6)} \neg (\predicate_2(\px)) \wedge \eventually_{[6,6]}(\predicate_1(\px)) \wedge \globally_{[6,6]}\neg (\predicate_2(\px)), 
        \\
        \Phi_3 =    & \globally_{[0,6]} \neg (\predicate_2(\px)) \wedge \eventually_{(6,18]}(\predicate_1(\px)).
    \end{align*}
\end{example}

% \qh{Need to handle singletons}

\subsubsection{Parse Tree}

From a time partitioned formula $\varphi$, we can construct a parse tree $\mathcal{T}$ with $n$ branches, each corresponding to a $\Phi_i$, $i\in \{1,\ldots,n\}$. Without loss of generality, let subformula $\Phi_i$ 
be in the following form:
\begin{align}
    \label{eq:hybridautomata}
    \Phi_i = \psi_{\la 0,t_1 \ra}\wedge\psi_{\la t_1,t_2 \ra}\wedge\cdots\wedge\psi_{\la t_{m-1},t_{m} \ra}.
\end{align}
$\Phi_i$ can always be written in this form by aggregating subformulas with the same time interval. Then, in the branch of $\mathcal{T}$ corresponding to $\Phi_i$, there are 
% can be represented as a parse tree $\mathcal{T}_k$ with each of the 
$m$ nodes, each representing a time-partitioned subformula $\psi_{\la t_{j-1},t_j \ra}$ for $j \in \{1,\ldots,m\}$.
% and transitions to the next node $\psi_{(t_k, t_l]}$ corresponding to the next time window. The full parse tree $T$ is the composition of the sub-parse trees (or branches), i.e, $\mathcal{T}_i$ for $i \in \{1,\cdots, n\}$.
% , i.e., $t > t_k$ is a for transition to the node $\psi_{(t_k, t_l]}$.
\begin{example}[Parse Tree]
    \label{ex:parsetree}
    Consider the partitioned formula in Example~\ref{ex:subformulas}. 
    % again. From Example~\ref{ex:subformulas}, we have
    % \begin{equation*}
    %     \varphi := \Phi_1 \vee \Phi_2 \vee \Phi_3,
    % \end{equation*}
    % where
    % \begin{align*}
    %     \Phi_1 =    & \eventually_{[0,6]}(\predicate_1(\px)) \wedge \globally_{[0,6]}\neg (\predicate_2(\px)), \\
    %     \Phi_2 =    & \eventually_{[6,6]}(\predicate_1(\px)) \wedge \globally_{[6,6]}\neg (\predicate_2(\px)) \wedge \globally_{[0,6)} \neg (\predicate_2(\px)), \\
    %     \Phi_2 =    & \eventually_{(6,18]}(\predicate_1(\px)) \wedge \globally_{[0,6]} \neg (\predicate_2(\px))
    % \end{align*}
    Each $\Phi_i$ can be represented as a branch
    $\mathcal{B}_i = (\text{V}_i,E_i)$ consisting of a set of nodes $\text{V}_i$ and edges $E_i$:
    \begin{align*}
        \mathcal{B}_1 = & (\{\text{v}_{\psi^{1}_{[0,6]}}\}, \emptyset) \text{ from } \Phi_1,\\
        \mathcal{B}_2 = & (\{\{\text{v}_{\psi^{2}_{[0,6)}}, \{\text{v}_{\psi^2_{[6,6]}}\},\{(\{\text{v}_{\psi^{2}_{[0,6)}}, \{\text{v}_{\psi^2_{[6,6]}})\} \text{ from } \Phi_2,\\
        \mathcal{B}_3 = & (\{\{\text{v}_{\psi^{3}_{[0,6]}}, \{\text{v}_{\psi^3_{(6,18]}}\}, \{(\{\text{v}_{\psi^{3}_{[0,6]}}, \{\text{v}_{\psi^3_{(6,18]}})\}) \text{ from } \Phi_3.
    \end{align*}
    % \begin{align*}
    %     \mathcal{T}_1 = & (\{v_{\psi^{1}_{[0,6)}}\},\emptyset) \\& \text{ corresponding to } \eventually_{[0,6]}(\predicate_1(\px)) \wedge \globally_{[0,6]} \neg (\predicate_2(\px))\\
    %     \mathcal{T}_2 = & (\{v_{\psi^{2}_{[0,6]}}, v_{\psi^2_{[6,6]}}\},\{(v_{\psi^{2}_{[0,6]}}, v_{\psi^2_{[6,6]}})\} \\& \text{ corresponding to } \globally_{[0,6)} \neg (\predicate_2(\px)) \wedge \eventually_{[6,6]}(\predicate_1(\px))\\
    %     \mathcal{T}_3 = & (\{v_{\psi^{3}_{[0,6]}}, v_{\psi^3_{[6,18]}}\}, \{(v_{\psi^{3}_{[0,6]}}, v_{\psi^3_{[6,18]}})\}) \\& \text{ corresponding to } \globally_{[0,6]} \neg (\predicate_2(\px)) \wedge \eventually_{(6,18]}(\predicate_1(\px))
    % \end{align*}
    Then, the parse tree is $\mathcal{T} = (\text{V}_1 \cup \text{V}_2 \cup \text{V}_3, E_1 \cup E_2 \cup E_3)$ as shown in Fig~\ref{fig:parsetree}.
\end{example}

\begin{figure}[t]
    \centering
    \resizebox{0.4\linewidth}{!}{
    \begin{tikzpicture}[->,>=stealth]
    \node[circle, fill,scale=0.3] (s0) at(0,0) {};
      \node[state, above right= of s0] (q1) {$\psi^{1}_{[0,6]}$};
      \node[state, right = 0.5cm of s0] (q3) {$\psi^2_{[0,6)}$};
      \node[state, right = 0.5cm of q3] (q4) {$\psi^2_{[6,6]}$};
      \node[state, below right = of s0] (q5) {$\psi^3_{[0,6]}$};
      \node[state, right = 1cm of q5] (q6) {$\psi^3_{(6,18]}$};
        \draw (q3) edge[above] node{} (q4)
        (s0) edge[above] node{} (q1)
        (s0) edge[above] node{} (q3)
        (s0) edge[above] node{} (q5)
        (q5) edge[above] node{} (q6);
    \end{tikzpicture}
    }
    \caption{Parse Tree in Example \ref{ex:parsetree}.
    % \ml{open/close time bounds don't match with the one in $\mathcal{B}_i$}
    }
    \label{fig:parsetree}
    \vspace{-2mm}
\end{figure}

\subsubsection{Timed NFA Construction}
Now, consider a parse tree node corresponding to formula $\psi_{\la t_{j-1},t_{j} \ra}$. By ignoring the time interval 
% $[t_j, t_k]$
$\la t_{j-1},t_j \ra$, we obtain the untimed version of this formula, $\psi^{j}$. By using the labeling scheme described above to define atomic propositions on predicates, $\psi^{j}$ can be treated as an LTLf formula since (i) the evaluation of $\psi_{\la t_{j-1}, t_j \ra}$ is over the same time interval for all temporal operators in $\psi^{j}$ due to syntactic separation, and (ii) each time interval is finite. Therefore, if a timed path $(\mathbf{p}, \mathbf{t}) \models \psi_{\la t_{j-1},t_j \ra}$, then its untimed word $w(\mathbf{p}) \models \psi^{j}$.

Recall that an LTLf formula can be translated into a DFA with an equivalent language. Thus, we can translate $\psi^{j}$ to a DFA $\mathcal{A}_{j}$ (for every node of the parse tree). To respect the time interval of the original formula $\psi_{\la t_{j-1},t_j \ra}$, we add the time interval $\la t_{j-1},t_j \ra$ as an invariant to every state in $\mathcal{A}_j$, obtaining timed DFA $\TA_j$ with the set of symbols $2^\Predicate \times \mathbb{T}$.  
% Recall that, for an input ($\sigma, t$) where $\sigma \in 2^\Predicate$, the transition from state $q$ to $q'$ is only valid if $t \in \text{Inv}(q')$.

% To complete the construction of the automaton for each branch of $\mathcal{T}$, we combine the timed DFAs successively in order according to $\mathcal{T}$. To combine them, we add transitions from the accepting states of the timed DFA $TA_{j,k}$ if there exists an outgoing transition in the corresponding node $\psi_{[t_j,t_k)}$ in $\mathcal{T}$ to another node in $\mathcal{T}$. For instance, let there be a transition between two nodes in the parse tree, $\psi_{[t_j,t_k]}$ and $\psi_{(t_k,t_l]}$ where $t_j \leq t_k \leq t_l$. In the corresponding constructed timed DFAs $TA_{j,k}$ and $TA_{k,l}$, for each transition $(q_{0, kl}, \sigma_i) \rightarrow q$ from a start state $q_{0, kl}$ in $A_{k,l}$, we add the transition $(q_{a,jk}, \sigma_i) \rightarrow q$ to each accepting state $q_{a,jk}$ in $TA_{j,k}$. Finally, only the accepting states of the DFA translated from the last node $\psi_{(t_{m-1},t_{m}]}$ of the parse tree $T$ remain as accepting states in the combined automaton. Therefore, this gives us the timed NFA $\TA$, which may have multiple possible transitions for a given input $(\sigma, t)$.


To complete the construction of the automaton $\TA_\varphi$ for the original $\varphi$, we connect the states of the timed DFAs successively according to the edges in $\mathcal{T}$.  Let $\mathcal{A}_j$ and $\mathcal{A}_{j+1}$ be two DFAs corresponding to a parent and its child node $\mathcal{T}$, respectively.  Further, let $q^F_j$ be an accepting state of $\mathcal{A}_j$ and $q^0_{j+1}$ be the initial state of $\mathcal{A}_{j+1}$. We add a transition from $q^F_j$ to every successor of $q^0_{j+1}$ with the corresponding symbol in $2^\Gamma$. Finally, we define the accepting states of $\TA_\varphi$ using the accepting states of the DFAs corresponding to the leaf nodes of the parse tree $\mathcal{T}$ in the following way. If the accepting state of this DFA is an absorbing state, then the same corresponding state is accepting. If this state is not absorbing, we add a transition to a new absorbing accepting state $q^F_\varphi$ with the time interval ${\la t_f, \infty)}$ 
% \ml{typo?}
as an invariant, where $t_f$ is the right time bound of the previous accepting state. The resulting structure is $\TA_\varphi$, which is a single timed NFA due to the added transitions between the DFAs.

%  Finally, we define the accepting states of $\TA_\varphi$ to be the accepting states of the DFAs that corresponding to the leaf nodes of the parse tree $\mathcal{T}$.
% both transitions to states within the same DFA $D_{j,k}$ and transitions to states of the DFA $D_{k,l}$ after combination.

% \ri{this is a little hairy to keep track of, is there a way to have the automaton and accepting state use similar subscripts? ie accepting state of $D_{t_j,t_k}$ could be $a_{j,k}$ or $q_{a,jk}$ could be the accepting state of DFA $D_{jk}$ operating in bounds $[t_j,t_k].$ just suggestions but it's hairy right now}
% Formally, we define the hybrid automaton as $\mathcal{H} = (Z, \Sigma, Inv, R)$. The set of discrete states $Z$ is the collection of all the states of the DFAs for the parse tree branch, giving us a one-to-one relation between the nodes in $\mathcal{T}$ and the states of $\mathcal{H}$. Inv($z$) is the time interval of the parse tree node that the DFA state is constructed from. The set of inputs is the power set of predicates, i.e., $\Sigma = 2^\Predicate$. The transition relation is as follows. For an input $\sigma \in \Sigma$, the transition $(z_i, (\sigma \wedge (t \in Inv(z_j)))) \rightarrow z_j$ exists in $H$ if the transition $(z_i, \sigma) \rightarrow z_j$ exists in the collection of DFAs. Additionally, we add transitions from the accepting states of DFA $D_{j,k}$ if there exists an outgoing transition in the corresponding node $\psi_{[t_j,t_k)}$ in $\mathcal{T}$. For instance, let there be a transition between two nodes in the parse tree, $\psi_{[t_j,t_k)}$ and $\psi_{[t_k,t_k)}$. In the corresponding constructed DFAs $D_{j,k}$ and $D_{k,l}$, for each transition from the start state $z_0$ in $D_{k,l}$, $(z_0, \sigma_i) \rightarrow z$, we add the transition $(z_{a}, (\sigma_i \wedge (t \in Inv(z))) \rightarrow z$ to each state $z_{a}$ of $H$, where $z_{a}$ refers to the accepting state of $D_{j,k}$. The accepting states of the DFA translated from the last node $\psi_{[t_{n-1},t_{n})}$ of the parse tree $T$ becomes the accepting states of $\mathcal{H}$. Therefore, $\mathcal{H}_{\Phi_1}$ is the hybrid automaton for the branch of $\mathcal{T}$ corresponding to subformula $\Phi_1$, a 'sequence' of LTLf-induced DFAs corresponding to each time-partitioned sub-subformula.

% Finally, we construct an untimed transition version of $\mathcal{H}_{\Phi_1}$, by ignoring time in the state transitions, to obtain an NFA $\mathcal{N}_{\Phi_1}$. By ignoring time in the transitions, there may be multiple transitions for a given symbol, both transitions to states within the same DFA $D_{j,k}$ and transitions to states of the DFA $D_{k,l}$ corresponding to the next sub-subformula.

% \qh{Check abuse of open and closed intervals for the time intervals.}

\begin{example}
 \label{ex:hybridautomaton}
Consider subformula 
    $\Phi_3 = \globally_{[0,6]} \neg (\predicate_2(\px)) \wedge \eventually_{(6,18]}\predicate_1(\px))$ from Example~\ref{ex:subformulas}. Using \eqref{eq:hybridautomata}, we obtain
    \begin{align*}
        \psi^3_{[0, 6]} = \globally_{[0,6]} \neg (\predicate_2(\px)), \\
        \psi^3_{(6,18]} = \eventually_{(6,18]}(\predicate_1(\px)).
    \end{align*}
    We translate each $\psi$ to an LTLf formula by evaluating the untimed version of $\psi$:
    \begin{align*}
        \psi^{0,6} = \globally \neg (\predicate_2(\px)), \\ %\label{eq: example psi06}, \\
        \psi^{6,18} = \eventually (\predicate_1(\px)), \\ % \label{eq: example psi618},
    \end{align*}
    and translate each LTLf formula into a DFA. The DFA for each LTLf formula is shown in Fig.~\ref{fig:dfa_0} and Fig. \ref{fig:dfa_6}.
    % To construct the final timed automaton $\TA_{\Phi_3}$, we duplicate the transitions for the starting state of the DFA translated from $\psi^{6,18}$ into the transitions of the accepting state of the DFA translated from $\psi^{0,6}$. This gives us the automaton depicted in Fig~\ref{fig:dfa} (c).
    The final timed automaton $\TA_{\Phi_3}$ is show in Fig. \ref{fig:final_TA}.
\end{example}

\begin{figure}[t]
  \begin{center}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \begin{tikzpicture}[->,>=stealth]
      \node[state, initial, accepting] (q1) {$q_1$};
        \draw (q1) edge[loop above] node{$\neg\predicate_2$} (q1);
    \end{tikzpicture}
    \caption{DFA for $\psi^{0,6}$ 
    \label{fig:dfa_0}
    % = \globally \neg (\predicate_2(\px))$.
    }
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
      \begin{tikzpicture}[->,>=stealth]
      \node[state, initial] (q1) {$q_1$};
        \node[state, accepting, right= 1cm of q1] (q2) {$q_2$};
        \draw (q1) edge[loop above] node{$\neg \predicate_1$} (q1)
        (q1) edge[above] node{$\predicate_1$} (q2)
        (q2) edge[loop above] node{$\top$} (q2);
    \end{tikzpicture}
    \caption{DFA for $\psi^{6,18}$
    \label{fig:dfa_6}
    % = \eventually (\predicate_1(\px))$.
    }
    \vspace{2mm}
    \end{subfigure}
    % \newline
    % \begin{subfigure}{\linewidth}
    %         \centering
    %         \begin{tikzpicture}[->,>=stealth]
    %         \node[state, initial] (q1) {\shortstack{$z_1$\\ $t \in [0, 6)$}};
    %         \node[state, right = 2.5cm of q1] (q2) {\shortstack{$z_2$\\ $t \in [6, 18]$}};
    %         \node[state, accepting, below = of q2] (q3) {\shortstack{$z_3$\\ $t \in [6, 18]$}};
    %         \draw (q1) edge[loop above] node{$\neg\predicate_2 \wedge t \in [0,6)$} (q1)
    %         (q1) edge[above] node{$\neg \predicate_1 \wedge t \in [6,18]$} (q2)
    %         (q1) edge[bend right, below] node{$\predicate_1 \wedge t \in [6,18]$} (q3)
    %         (q2) edge[loop above] node{$\neg \predicate_1 \wedge t \in [6,18]$} (q2)
    %         (q2) edge[above] node{$\predicate_1 \wedge t \in [6,18]$} (q3)
    %         (q3) edge[loop below] node{$\top$} (q3);
    %         \end{tikzpicture}
    %         \caption{Timed hybrid automaton $\mathcal{H}_{\Phi_3}$ for Example~\ref{ex:hybridautomaton}. Node $z_1$ corresponds to the DFA (a), while nodes $z_2$ and $z_3$ correspond to the DFA (b).}
    %     \end{subfigure}
    \newline
    \begin{subfigure}{.9\linewidth}
            \centering
            \scalebox{0.6}{
            \begin{tikzpicture}[->,>=stealth]
            \node[state, initial] (q1) {\shortstack{$q_1$\\ $t \in [0, 6]$}};
            \node[state, right = 2.5cm of q1] (q2) {\shortstack{$q_2$\\ $t \in (6, 18]$}};
            \node[state, accepting, below = of q2] (q3) {\shortstack{$q_3$\\ $t \in (6, 18]$}};
            \draw (q1) edge[loop below] node{$\neg\predicate_2$} (q1)
            (q1) edge[above] node{$\neg \predicate_1$} (q2)
            (q1) edge[bend right, below] node{$\predicate_1$} (q3)
            (q2) edge[loop right] node{$\neg \predicate_1$} (q2)
            (q2) edge[right] node{$\predicate_1$} (q3)
            (q3) edge[loop right] node{$\top$} (q3);
            \end{tikzpicture}
            }
            \caption{Timed NFA for Example~\ref{ex:hybridautomaton}. State $q_1$ corresponds to the DFA in (a) and $q_2$ and $q_3$ correspond to the DFA in (b).}
            \label{fig:final_TA}
        \end{subfigure}
    \caption{NFA construction from STL formula $\Phi_3 = \globally_{[0,6]} \neg (\predicate_2(\px)) \wedge \eventually_{(6,18]}(\predicate_1(\px))$.}
    \label{fig:dfa}
  \end{center}
   \vspace{-2mm}
\end{figure}

The following theorem states that the constructed timed automaton accepts precisely the timed words of the trajectory that satisfy $\varphi$.
\begin{theorem} 
\label{theorem:timedsatisfiesstl}
A trajectory (timed path) is accepted by the timed NFA $\TA_\varphi$ if and only if it satisfies \stlnn formula $\varphi$.
\end{theorem}
\begin{proof}[Proof Sketch]
    We prove $\rightarrow$, but $\leftarrow$ is proven in a similar manner. Let $\varphi'$ be the syntactically separated formula for $\varphi$, using the minimal time partitioning set $\mathbf{T}_0$ (although a larger time partitioning does not change the result). In DNF, $\varphi' = \Phi_1 \vee \Phi_2 \vee \cdots \vee \Phi_n$. Without loss of generality, consider $\Phi_k$, a branch of the parse tree where $\Phi_k = \psi_{\la 0,\tau_1 \ra}\psi_{\la \tau_1,\tau_2 \ra}\cdots\psi_{\la \tau_m-1, \tau_m \ra}$. Let any timed word $w$ that is accepted by $\TA_{\Phi_k}$ be $(L(x_0), t_0)(L(x_1), t_1)\cdots(L(x_n), t_n)$. By separating this timed word into segments using $\mathbf{T}_0$, we obtain a set of subsequences of the timed word (sub-word) of the general form $(L(x_j), t_j)\cdots(L(x_k), t_k)$, where $\tau_{j} \leq t_j \leq t_k \leq \tau_{k}$ for the time window $\la \tau_{j}, \tau_{k}\ra$. Through minimal time partitioning, we are guaranteed to have all temporal operators in $\psi_{\la \tau_j, \tau_k \ra}$ have the same time window $\la \tau_j, \tau_k \ra$. Therefore, the sub-word within this partition satisfies $\psi_{\la \tau_i, \tau_k \ra}$, as this sub-word is accepted by the LTLf translated from $\psi_{\la \tau_i, \tau_k \ra}$. Doing the same for all sub-words in the partition set gives us the result that any trajectory $\mathbf{x}$ that produces this complete timed word satisfies the full formula $\varphi$.
\end{proof}
% \reviewer{ I am wondering how the labelling function defined for
% the times paths (Def 7) can be guaranteed. It seems like
% the way of defining it lacks of robustness and has
% something to do with the nonlinearities in the concrete
% dynamics. It would be great to add a short remark to explain
% how this works.}

\subsection{Product Automaton}

The final structure used for high-level discrete search is a product automaton $\mathcal{P}$, which captures all possible ways that paths can satisfy $\varphi$. The product automaton is computed as $\mathcal{P} = \TA_\varphi \otimes \mathcal{M}$ (Line 3 of Alg.~\ref{alg:framework}). $\mathcal{P}$ is a tuple $(Z, Z_0, \delta_p, \text{Inv}_p, F_p)$, where

\begin{itemize}
    \item $Z = Q \times D$;
    \item $\delta_p : Q \times D \rightarrow Q \times D$, such that $(q', d') \in \delta_p(q, d)$ if $(d, d') \in E$ and $q' \in \delta(q, L(d))$;
    \item $\text{Inv}: Q \times D \rightarrow \mathcal{I}$, such that  $\text{Inv}((q,d)) = \text{Inv}(q)$;
    \item $F_p = F \times D$.
\end{itemize}

We refer to state $z = (q,d) \in Z$ of $\mathcal{P}$ as a high-level state. 
% $\mathcal{P}$ is a directed graph, in which there exists an edge from the high-level state $(d, q)$ to $(d', q')$ if there exists a transition both from $d$ to $d'$ in $\mathcal{M}$ and $q$ to $q'$ in $\TA_{\phi}$. 
State $z$ inherits the invariant of its automaton state $q$. State $z$ is accepting if $q \in F$ is an accepting state.
Every accepting run of $\mathcal{P}$ is a sequence of high-level states, $(q_0, d_0)(q_1, d_1)\cdots(q_p, d_p)$. A continuous trajectory that follows the sequence of regions $d_0d_1\cdots d_p$ and respects the invariant constraints of $q_0q_1\cdots q_p$ satisfies $\varphi$. 

% By ignoring time, there may be multiple transitions for a given symbol, both transitions to states within the same DFA $D_{j,k}$ and transitions to states of the DFA $D_{k,l}$ corresponding to the next sub-subformula.\qh{rewrite this for product automaton}

% Note that the product automaton does not handle time explicitly ina

\subsection{Time Partitioned Automaton-guided Search}
\label{sec:planning}
% \qh{why not parallelize it if we have disjoint branches?}
To generate a satisfying trajectory, we extend the co-safe LTL planning framework in \cite{Bhatia2010, Maly2013} to include time window constraints.
The framework consists of two main layers: an automaton-based high-level search layer and a low-level sampling-based planner. 
% For temporal logic planning problems, interplay between discrete search and continuous state-space exploration has been shown to improve the efficiency of finding solutions \cite{Maly2013}. 
% Our planning framework is similar to the framework discussed in past works \cite{Maly2013,pastworks2}, with modifications to handle time windows.

\subsubsection{High-level layer}
\label{sec:highlevel}
In each iteration of high-level planning, the high-level layer searches the product automaton $\mathcal{P}$ constructed above. By searching $\mathcal{P}$, an accepting run (called lead) $\mathbf{L}$ is computed at each iteration. Each lead is a
candidate sequence of contiguous high-level states through
which the algorithm attempts to guide a sampling-based motion tree of continuous trajectories in the low-level layer. A graph search algorithm, such as Dijkstra's Algorithm, is used to find the shortest path to an accepting state from a start state according to the following edge weight computation. For each high-level state $(q,d)$, we propose to assign a weight defined by
\begin{align}
    w(d,q) = \frac{(cov(q,d) +1)\cdot vol(d) \cdot duration(q)}{DistFromAcc(q) \cdot (numsel(q,d) +1)^2},
\end{align}
where $cov(q,d)$ is the number of motion tree vertices in the state $(q,d)$, $vol(d)$ is the estimated volume of the state space covered by abstraction region $d$, $duration(q)$ is size of the time interval associated with automaton state $q$, $DistFromAcc(q)$ is the shortest unweighted path from the automaton state $q$ to an accepting state in $\TA_\varphi$, and $numsel(q,d)$ is the number of times the high-level state ($d,q$) has been selected for expansion. The edge weight between two states is then defined as:
\begin{align}
    w((q_1,d_1),(q_2,d_2)) = \frac{1}{w(q_1,d_1)\cdot w(q_2,d_2)}.
\end{align}
These weights are updated in every iteration. Such a weighting scheme has been shown to promote expansion in unexplored areas (i.e., where $cov$ and $numsel$ are both small) and to suppress expansion in areas where attempts at exploration have repeatedly failed (i.e., where $numsel \gg cov$) \cite{Maly2013}.
% \reviewer{- Section IV.D-1: vol(d) seems to be difficult to compute.
% How good must the approximation be?}
% \reviewer{-What is the intuition to positively consider the volume of
% a partition to define the cost of a high-level state?
% }
% \ri{is this the LTL weighting scheme? If so, we can consider cutting this out and referencing that paper if we need to start saving space. or we should at least cite it for "it has been shown.."}
\subsubsection{Low-level layer - Incorporating Time Constraints}

\begin{algorithm}
    \caption{Explore}
    \label{alg:explore}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{Lead $\mathbf{L}$, set of high-level states $C$, motion tree $\textsc{tr}$, product automaton $\mathcal{P}$, State Space $X$, exploration time $t_{e}$,}
    \Output{Solution trajectory of tree nodes containing system state, and high-level states $(\mathbf{v},\mathbf{t})$ ending with $v$, and its controller $\pu$, if one is found; return NULL otherwise.}
    \While{Time Elapsed $< t_e$}
    {
        $(d,q) \leftarrow$ C.sample()\\
        $v_s \leftarrow $ Sample(d,q)\\
        $v \leftarrow $ SelectAndExtend($\mathcal{P}, \textsc{tr}, v_s, X$)\\
        \If{isValid($v$)}{
        Add vertex $v$ to \textsc{tr}\\ 
        \If{isAccepting($v.q$)}{
            $(\mathbf{v},\mathbf{u}, \mathbf{t})  \leftarrow$ Extract trajectory ending with $v$ and control inputs from \textsc{tr}\\
            \Return $(\mathbf{v}, \pu, \mathbf{t})$
        }
        \If{$(v.d, v.q) \notin C \wedge (v.d, v.q) \in L$}
        {
            $C \leftarrow C \cup \{(v.d, v.q)\}$
        }
        }
    }
    \Return $\emptyset$
\end{algorithm}
% \qh{REWRITE LOW LEVEL PLANNER}
% \reviewer{With view to the actual control synthesis, i.e., the
% controller that steers the system from one automaton state
% to the next, is rather vague. This is only a minor
% criticism as the paper focuses on the planning part. Nevertheless, as the authors emphasize in the introduction that general nonlinear systems can be handled by the
% proposed algorithm, some more system theoretic details
% would be interesting. In particular in Section IV.D-2, the
% authors refer to a motion tree without providing a
% reference or details on its construction. Are
% state-feedback controllers employed with finite-time
% convergence? Is a continuous or discrete-time controller
% used? These questions are important in order to ensure that
% also the real controlled system satisfies the STL
% specifications.
% }
% The low-level layer utilizes a tree-based motion planning framework that is able to handle dynamics and kinematic constraints of the system while avoiding collisions. By following the high-level lead $\mathbf{L}$, the real system is ensured to satisfy the STL specification if a solution is found.
Given a lead $\mathbf{L}$, we compute the set of high-level states $C$ that exist in $\mathbf{L}$ and contain at least one vertex of a motion tree (line 7 of Alg.~\ref{alg:framework}). The low-level search promotes tree expansion in the high-level states of $C$ (Alg.~\ref{alg:explore}). In each iteration of low-level planning, a high-level state $z$ is sampled from $C$ with probability proportional to the weights of each high-level state in $C$. A tree vertex $v_s$ is then sampled within $z$, and one iteration of tree-search motion planning is performed to obtain a new tree vertex $v_n$. A tree vertex is a tuple $v = (x, q, d, t)$. An iteration of tree-search motion planning involves selecting a tree vertex $v_{sel}$, sampling a valid control $u \in U$ and time duration, and propagating the dynamics \eqref{eq:system} of the continuous state component $x_{sel}$ of $v_{sel}$ using numerical propagation techniques (e.g., Runge-Kutta methods) to obtain a new continuous state component $x_n$ and time $t_n$. Any tree-based motion planner that supports kinodynamic constraints can be used at this step, such as RRT \cite{kinorrt} or EST \cite{EST}. The new discrete state components $q_n, d_n$ of $v_n$ are obtained by propagating the product automaton $\mathcal{P}$.

Vertex $v$ is valid if both its continuous and discrete state components are valid. The continuous component $v.x$ is valid if it obeys the state constraints of System~\eqref{eq:system}. Our main addition to the existing multi-layered planner is the handling of time constraints in this low-level layer. The discrete components $v.q$ and $v.d$ are valid if $(v.q,v.d)$ exists in the product automaton and the vertex time $v.t$ is in the invariant of $v.q$, i.e., $v.t \in \text{Inv}(v.q)$. Without considering the time component, a newly extended vertex of the motion tree may have multiple possible discrete components (high-level state) due to the non-determinism of $\TA$. The time component determines the valid high-level state.

Suppose that a new vertex $v_n$ corresponds to a newly reached high-level state that is in the current discrete lead $\mathbf{L}$, this high-level state is added to the set of available states for exploration $C$. Finally, if the automaton state $v_n.q$ is an accepting state, the trajectory ending with $v_n$ and its corresponding controller $\pu$ is returned as a solution.

% \begin{remark}
% The satisfaction of an STL formula is defined based on dense continuous time. For example, the formula $\globally_{[0,2]} (x > 0) \wedge \globally_{[2,4]}(y > 0)$ requires that $x > 0$ for the continuous time interval $[0,2]$ and $y>0$ for the interval $[2,4]$. However, sampling-based algorithms (including the one proposed this work) perform in discrete time, even with interpolation between discrete points. To reconcile this issue with discrete-time algorithms, we define a relaxation, dubbed as $\epsilon-$robust satisfaction, which refers to $\epsilon$ resolution of time discretization.  \ml{we still need to work out the detail of this.}

% \begin{definition}[$\epsilon-$Robust Satisfaction]
%     A trajectory $\epsilon-$robustly satisfies an \stlnn formula $\varphi$ if there does not exist any $\delta > \epsilon$ such that the trajectory at the interval $[t, t + \delta]$ does not satisfy $\varphi$.
%     \ml{need to polish this... it's unclear}
% \end{definition}

% In this paper,  on $\epsilon-$satisfaction instead of dense-time satisfaction.
% \end{remark}


==> sections/camera_ready/Analysis.tex <==
\section{Correctness and Completeness}

% In this section, we show that our framework is sound and probabilistically complete \footref{footnote_extendedversion}.
The following lemma provides the correctness guarantee of the proposed framework.  That is, the returned trajectory by the algorithm is guaranteed to satisfy $\varphi$.

\begin{lemma}[Correctness]
\label{lemma:correctness}
Given a lead $\mathbf{L}$ computed by $\mathcal{P}$, $\exists \mathbf{t} = t_0t_1\cdots t_l$ associated with $\mathbf{L}$ that produces a timed word $(\mathbf{w}, \mathbf{t})$ such that any trajectory that realizes this timed word satisfies STL$_{nn}$ formula $\varphi$.
\end{lemma}
% \begin{proof}[Proof Sketch]
%     Observe that $\TA_\varphi$ is an NFA with time constraints.
%     The proof is straightforward from the definition of the language of the NFA corresponding to $\TA_\varphi$ and Theorem~\ref{theorem:timedsatisfiesstl}. Consider a lead $\mathbf{L}$ that produces a word $\mathbf{w}$, through the sequence of regions $\mathbf{d}$, accepted by $\mathcal{P}$. Since $\mathcal{P}$ is a Cartesian product of $\TA_\varphi$ and $\mathcal{M}$, the set of words that are accepted by $\mathcal{P}$ is a subset of the language of the NFA. Therefore, this word can be converted to a timed word $(\mathbf{w}, \mathbf{t})$ that is accepted by $\TA_\varphi$. By Theorem~\ref{theorem:timedsatisfiesstl}, all trajectories that realizes this timed word necessarily satisfies $\varphi$.
%     \vspace{-1mm}
% \end{proof}
\noindent
% See the extended version \cite{CDC22extendedversion} for the proof of Lemma~\ref{lemma:correctness}.
% Lemma~\ref{lemma:correctness} provides the correctness guarantee of the proposed framework.  That is, the returned trajectory by the algorithm is guaranteed to satisfy $\varphi$. 
The algorithm is also probabilistically complete, as given by the theorem below.
% Since $\mathcal{P}$ is a cartesian product of $\TA$ and the transition system $\mathcal{M}$, the language of $\mathcal{P}$ is the untimed language of $\TA$.\qh{check if this claim is true}
% Lemma~\ref{lemma:correctness} provides a useful property of $\mathcal{P}$ for controller synthesis. Given a path of high-level states $\mathbf{z}$ accepted by $\mathcal{P}$, we can find a timed path using the fact that $\mathbf{z}$ can be seen as a valid set of untimed discrete waypoints for a trajectory in order to satisfy $\varphi$. This means that for the product automaton, the lead  computed by the high-level planner is guaranteed to be a correct discrete path.
% Lemma~\ref{lemma:correctness} provides the correctness guarantee of the proposed framework.  That is, the returned trajectory by the algorithm is guaranteed to $\epsilon$-satisfy $\varphi$. 
\begin{theorem}[Probabilistic Completeness]
    \label{theorem:completeness}
    Alg.~\ref{alg:framework} is probabilistically complete, i.e., Alg.~\ref{alg:framework} finds a satisfying solution if one exists almost surely as time approaches infinity.
\end{theorem}
\noindent
The proofs of Lemma~\ref{lemma:correctness} and Theorem~\ref{theorem:completeness} are in the extended version of this work \cite{CDC22extendedversion}.
% \begin{proof}[Proof Sketch]
%     The proof of probabilistic completeness follows from the probabilistic completeness of the tree search based algorithm. In each iteration of high-level planning discrete search of the product automaton computes a lead, which is a valid candidate series of high-level regions by Theorem~\ref{lemma:correctness}. For the low-level layer, the probability of finding a continuous trajectory solution that obeys the invariant constraints according to a given lead, if one exists, approaches $1$ as $t_e \rightarrow \infty$. Since the edge weights of the product automaton are updated every iteration, the probability of searching all possible solution paths in $\mathcal{P}$ approaches $1$ as well. By iterating between high-level and low-level planning, the algorithm produces continuous trajectories covering the entire search space with probability $1$ as $t_{\max} \rightarrow \infty$.
% \end{proof}
% \qh{Probabilistic completeness with respect to sampling, from paper: Simulation frameworks typically provide signal values at discrete time instants, usually this is a by-product of using a numerical technique to solve the differential equations in the underlying system. These discrete-time solutions are assumed to be sampled versions of the actual signal, which can be reconstructed using some form of interpolation.}

==> sections/camera_ready/Conclusion.tex <==
\section{Conclusion}

This paper proposes an algorithmic framework for automaton-guided control synthesis under STL specifications, for both nonlinear dynamics and predicates. The proposed framework is correct by construction and probabilistically complete, and empirical evaluation demonstrates its effectiveness and efficiency. Additionally, we plan to consider dynamics and measurement uncertainty by incorporating tree-search approaches such as in \cite{ho2022gbt}, which would allow such control systems to be more readily applied in real world scenarios.

% For future work, a natural extension is to generalize our approach to nested STL specifications. Additionally, we plan to consider dynamics and measurement uncertainty by incorporating tree-search approaches such as in \cite{ho2022gbt}, which would allow such control systems to be more readily applied in real world scenarios.

% Finally, probabilistic guarantees on STL satisfaction under uncertainty could be done by considering belief space... Belief space (Gaussian Belief Trees), general POMDPs, bounded noise.

% \ri{are these ideas for future work? one could be to use a different weighting scheme for high level search (15,16) that takes advantage of STL quirks (like online monitoring) but please ignore if i'm way off the mark with that one}

%Future work includes online monitoring with multi-layered planning could also improve the effectiveness of the algorithm.

% However, for general STL specifications, the number of clocks can be very high \qh{unbounded?}, leading to an unclear way of handling clocks for synergistic planning.

==> sections/contributions.tex <==
Coherent difference between zone automaton and our automaton

provide a construction directly from specification, rather than through timed automaton -> zone automaton.

Claim: benefits of time partitioning through syntactic separation (larger and smaller discretization benefits).

Constructing automaton that is compatible with existing methods of motion planning.

probabilistic completeness, nonlinear dynamics.

polynomial predicates.

tweaking of motion plan to handle time

==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
In this section, we formally define concepts that are used in our approach.
% \subsection{Linear Temporal Logic with finite words ($LTL_{f}$)}
We use \textit{LTL with finite traces} (LTLf) in the construction of the automaton from \stlnn formulas.
\begin{definition}[LTLf Syntax]
    Let $P$ be a set of atomic propositions. Then, LTLf syntax is recursively defined by:
    \begin{align*}
        \psi := p \mid \neg \psi \mid \psi \wedge \psi \mid \tempop{X} \varphi \mid \psi \until \psi
    \end{align*}
    where $p \in P$, $\tempop{X}$ is the \textit{next} operator, and $\until$ is the until operator.
\end{definition}

The semantics of LTLf are defined over finite words.

\begin{definition}[LTLf Semantics]
    Given a finite word $\pi \in (2^P)^* $, denote by $|\pi|$ and $\pi_i$ the length of $\pi$ and the symbol in the $i^{th}$ position in $\pi$, respectively.  Then, 
    \begin{itemize}
        \item $\pi, i \models p \iff p \in \pi_i$:
        \item $\pi, i \models \psi \iff 0 \leq i \leq |\pi| \text{ and } \pi,i \models \psi$;
        \item $\pi, i \models \neg \psi \iff \pi, i \not\models \psi$;
        \item $\pi, i \models \psi \wedge \psi' \iff \pi, i \models \psi \text{ and } \pi, i \models \psi'$;
        \item $\pi, i \models \tempop{X} \psi \iff 0 < i < |\pi| - 1 \text{ and } \pi, i + 1 \models \psi$;
        \item $\pi, i \models \psi \until \psi' \iff \exists j \in \mathbb{N} \; \text{ s.t. } i \leq j \leq |\pi|$, we have $\pi, j \models \psi' \text{ and } \forall k, i \leq k < j, \text{ we have } \pi, k \models \psi$.
    \end{itemize}
\end{definition}
\noindent 
% The \textit{language} of a formula $\psi$ denoted by $\mathcal{L}(\psi)$ is the set of all words that satisfy $\psi$, i.e.,  $\mathcal{L}(\psi) = \{\pi \in (2^P)^* \mid \pi \models \psi\}$.

We utilize non-deterministic finite automata (NFA) to guide sampling-based search.

\begin{definition}[NFA]
    \label{def:NFA}
    A non-deterministic finite automaton (NFA) is a tuple $\mathcal{A} = (Q, Q_0, \Sigma,  \delta, F)$, where
    \begin{itemize}
        \item $Q$ is a finite set of states;
        \item $Q_0 \subseteq Q$ is the set of initial states;
        \item $\Sigma$ is a set of input symbols;
        % , where each input symbol is a truth assignments to the propositions in $P$;
        \item $\delta : Q \times \Sigma \rightarrow 2^Q$ is the transition function;
        \item $F \subseteq Q$ is the set of accepting states.
    \end{itemize}
\end{definition}

% A finite run of $\mathcal{A}$ is a sequence of states $w = w_0w_1\cdots w_n$, where $w_0 = z_0$...\qh{todo} $w$ is an accepting run if $w_n \in F$. An input word that realizes an accepting run satisfies $\varphi$. The language $\mathcal{L}(A)$ of a NFA/DFA A is the set of input words that realizes accepting runs.\qh{This is wrong.}
\noindent
Given a finite word $\pi = \sigma_1 \sigma_2 \ldots \sigma_n$ where $\sigma \in \Sigma$, a run $q = q_0q_1\ldots q_n$, where $q_0 \in Q_0$ and $q_{i+1} \in \delta(q_i, \sigma_{i+1})$ for all $0\leq i<n$, on NFA $\mathcal{A}$ is induced.  We say $\pi$ is accepted by $\mathcal{A}$ if there exists an induced run $q$ such that $q_n \in F$.  The \textit{language} of $\mathcal{A}$ denoted by $\mathcal{L}(\mathcal{A})$ is the set of words that are accepted by $\mathcal{A}$.

A \textit{deterministic finite automaton} (DFA) is an NFA in which $|Q_0|=1$ and, $\forall q \in Q$ and $\forall \sigma \in \Sigma$, $|\delta(q,\sigma)| \leq 1$. 
% \begin{lemma}[Section 2 in~\cite{ltlf2dfa}]
%     Any LTLf formula $\psi$ can be algorithmically translated to a DFA $D_\psi$, such that $\mathbf{w} \models \psi \iff \mathbf{w} \in \mathcal{L}(D_\psi)$.
% \end{lemma}
Every LTLf formula $\psi$ defined over $P$ can be algorithmically translated to a DFA $\mathcal{A}_\psi$ with symbols $\Sigma = 2^P$ such that $\pi \models \psi \iff \pi \in \mathcal{L}(\mathcal{A}_\psi)$.

From \stlnn formulas, we construct an NFA that is constrained with time.
\begin{definition}[Timed NFA]
A timed NFA is a tuple $\TA = (Q, \Sigma_t, Q_0, \text{Inv}, \delta, F)$ where $Q, Q_0, \delta$ and $F$ are as in Def~\ref{def:NFA}, and
    \begin{itemize}
        \item $\Sigma_t = \Sigma \times \mathbb{T}$ is the set of input symbols,
        % input alphabet, 
        where each symbol in $\Sigma_t$ is a pair of $\sigma \in \Sigma$ and time $t \in \timedomain$;
        \item $\text{Inv} : Q \rightarrow \mathcal{I}$ is an invariant function over a (closed or open) interval of time, where $\mathcal{I}$ is the set of all intervals over $\mathbb{T}$;
    \end{itemize}
\end{definition}
\noindent
In $\TA$ a transition $q \xrightarrow{(\sigma, t)} q'$ exists iff $q' \in \delta(q, \sigma)$ and $t \in \text{Inv}(q')$.

% \subsection{Hybrid System}

% A hybrid system is defined as a tuple $\mathcal{H} = (Z, z_0, INV, E, Guard, Jump, U, Flow, \Pi, L)$, where

% \begin{itemize}
%     \item $S = Z \times X$ is the hybrid state space that is a product of a set of discrete modes, $Z = \{z_1, z_2 \cdots z_m\}$ for some finite $m \in \mathbb{N}$, and a set of continuous state space $X = \{X \subseteq \realnumbers^n\}$;
%     \item $s_0 \in S$ is the initial state;
%     \item Inv is the set of invariants;
%     \item $E \subseteq Z \times Z$ is the discrete transition between modes in $Z$;
%     \item $Flow = \{Flow_z : z \in Z\}$, where $Flow_z = X_z \times U_z \times \realnumbers^{\geq 0} \rightarrow X_{z}$ describes the continuous dynamics of the system through a set of differential equations
%     \item \qh{Incomplete}
% \end{itemize}

% \begin{definition}[Labeling function]
%     A labeling function $L: X \rightarrow \Sigma$ maps a state $x$ to an input symbol $\sigma$.
% \end{definition}

\begin{definition}[Timed path]
    Let $L: X \rightarrow \Sigma$ be a labeling function that maps a state $x  \in X$ to an input symbol $\sigma \in \Sigma$.
    A finite trajectory $\px$ in a state space $X$ defines a timed path $(\mathbf{p}, \mathbf{t}) = (x_0, t_0)(x_1, t_1)\cdots(x_l,t_l)$ such that for all $i \in \{0, \cdots, l\}$:
    \begin{itemize}
        \item $\mathbf{p} = x_0x_1\cdots x_l$, with $x_i = \px(t_i)$,
        \item $t_0t_1\cdots t_l$ is a sequence of time stamps, with $t_i \in \timedomain$ and $t_{i+1} \geq t_{i}$,
        \item $L(x_i)$ remains constant during the time interval $(t_i, t_{i+1})$, i.e., $L(\px(t)) = L(x_i)$ $\forall t \in (t_i,t_{i+1})$.
    \end{itemize}
\end{definition}

\begin{definition}[Timed word]
    A finite trajectory $\px$ with a timed path $(\mathbf{p}, \mathbf{t})$ generates a timed word $w(\px) = w((\mathbf{p}, \mathbf{t})) = (L(x_0), t_0)(L(x_1), t_1)\cdots(L(x_l),t_l)$.
\end{definition}

\noindent
% A run $\pi$ of a timed NFA $\TA$ with initial state $q_0$ over a timed word is a finite sequence of transitions $(q_0) \xrightarrow{\sigma_1, t_1} (q') \xrightarrow{\sigma_2, t_2}\cdots (q'')$. A timed word $w(\px)$ is accepted by $\TA$ if there exists an accepting run $\pi$ over $\TA$ such that the last state is accepting. 
% Similar to NFAs, a time word induces a set of runs on $\TA$, and $\TA$ accepts it if 
The notions of acceptance and language of $\TA$ over timed words are extended from NFAs in a straightforward manner.  In addition, we say that a timed path is accepted by $\TA$ if its timed word is accepted by $\TA$.



% \begin{definition}[Language]
%     The language $\mathcal{L}(\TA)$ is the set of all accepted timed words by $\TA$. 
% \end{definition}

% \begin{definition}[Untimed Language]
%     An untimed language of a timed DFA/NFA $\TA$, $\mathcal{L}_{un}(\TA)$, is the set of all untimed words accepted by $\TA$, by projecting the accepted timed words of $\TA$ onto their first components.
% \end{definition}


% \begin{definition}
%     A timed word $wt = (w, \mathit{I})$ is a pair that consists of a word and an interval sequence $\mathit{I}$.
% \end{definition}

% STL signals are continuous in the general case, which means that they are evaluated in \textit{dense-time} (continuous time). STL can also be evaluated over \textit{discrete-time}, for example if the underlying system is a discrete-time stochastic system. In such cases, we evaluate STL formulas every time step, and we denote $\mathcal{L_{\delta}}(\varphi)$ as the language of STL formula $\varphi$ evaluated in discrete time at some $\delta_t$ per time step. By evaluating a signal word $s(t)$ over discrete time steps, we can treat it like an untimed word $w$.

% Its untimed language Lun(A) is the set of all untimed words
% accepted by A, which are the projections of the accepted
% words of A onto their first components


% \subsection{Time partitioning of STL}
% \label{subsec:timepartitioning}

% Note that, by nesting STL formulas, the time interval of the inner subformulas become relative to the outer-subformulas.  We refer to the inner-subformulas time frames as \textit{local time}, and the time frame for the outer-most formula as the \textit{global time}.
% For instance, consider formula 
% $$\phi = G_{[0,1]} (\predicate_1 \to \eventually_{[0,2]} \predicate_2).$$
% For the subformula $\phi_2 = \eventually_{[0,1]} \predicate_2$, the clock starts at zero as soon as $\predicate_1$ becomes true within $[0,1]$.  Say $\predicate_1(s(0.5)) = \top$.  Then, $\phi$ requires that $\exists t \in [0.5,2.5]$ s.t. $\mu_2(s(t)) = \top$.  In this example, the time frame that $\globally_{[0,1]}$ lives in is the global time, and the time frame that $\eventually_{[0,2]}$ lives in is the local time.

% Work \cite{boundedmodelchecking} proposes an extension to STL, called signal temporal logic with global time (STL-GT) that adds global time constraints. This allows for syntactic separation of a formula, which depends only on a disjoint part of the underlying time domain.  In that work, STL temporal operator $\until_I$ is extended to STL-GT operator $\until_I^K$, where $K$ is the global time.

% The main result we use in this work from \cite{boundedmodelchecking} is the \emph{Global Separation} of $U_{I}^K$ at time $\tau$, which is given by:
% \begin{multline}
%     \label{eq:global separation}
%     \varphi \until_{I}^K \varphi' \equiv \varphi \until_{I}^{K \cap [0,\tau)}\varphi'  \; \vee \\
%     (\globally^{< \tau}_{\geq 0} \varphi \wedge \globally^{=\tau}_{\geq 0}\varphi \wedge (\eventually_{I}^{K \cap \{\tau\}}\varphi' \vee (\globally^{> \tau}_{=0}\varphi)\until_{I}^{K \cap (\tau, \infty)}\varphi'))
% \end{multline}

% Given an STL formula, we use the above equivalence to obtain an equivalent STL-GT formula such that each of its subformulas only depend on a specified global time interval.  Examples of such time partitioning is provided in Section~\ref{sec:method}.
